Enumerating minimal dominating sets and variants in chordal bipartite graphs

Enumerating minimal dominating sets with polynomial delay in bipartite graphs is a long-standing open problem. To date, even the subcase of chordal bipartite graphs is open, with the best known algorithm due to Golovach, Heggernes, Kant\'e, Kratsch, Saether, and Villanger running in incremental-polynomial time. We improve on this result by providing a polynomial delay and space algorithm enumerating minimal dominating sets in chordal bipartite graphs. Additionally, we show that the total and connected variants admit polynomial and incremental-polynomial delay algorithms, respectively, within the same class. This provides an alternative proof of a result by Golovach et al. for total dominating sets, and answers an open question for the connected variant. Finally, we give evidence that the techniques used in this paper cannot be generalized to bipartite graphs for (total) minimal dominating sets, unless P = NP, and show that enumerating minimal connected dominating sets in bipartite graphs is harder than enumerating minimal transversals in general hypergraphs.

==> preamble.tex <==
% problem environment
\usepackage{tabularx}
\usepackage{environ}
\makeatletter
\newcommand{\problemtitle}[1]{\gdef\@problemtitle{#1}}% 
\newcommand{\problemparameter}[1]{\gdef\@problemparameter{#1}}% Store problem title
\newcommand{\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand{\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question
\NewEnviron{problemgen}{
\problemtitle{}\problemparameter{}\probleminput{}\problemquestion{}% Default input is empty
\BODY% Parse input
\par\addvspace{.5\baselineskip}
\noindent
\begin{tabularx}{\textwidth}{@{\hspace{\parindent}} l X c}
    \multicolumn{2}{@{\hspace{\parindent}}l}{\@problemtitle} \\% Title
    % \textbf{Parameter:} & \@problemparameter \\% Input
    \textbf{Input:} & \@probleminput \\% Input
    \textbf{Output:} & \@problemquestion% Output
  \end{tabularx}
  \par\addvspace{.5\baselineskip}
}

\NewEnviron{problemdec}{
\problemtitle{}\probleminput{}\problemquestion{}% Default input is empty
  \BODY% Parse input
  \par\addvspace{.5\baselineskip}
  \noindent
  \begin{tabularx}{\textwidth}{@{\hspace{\parindent}} l X c}
    \multicolumn{2}{@{\hspace{\parindent}}l}{\@problemtitle} \\% Title
    \textbf{Input:} & \@probleminput \\% Input
    \textbf{Question:} & \@problemquestion% Output
  \end{tabularx}
  \par\addvspace{.5\baselineskip}
}

\def\lemmaautorefname{Lemma}
\def\sectionautorefname{Section}
\def\propositionautorefname{Proposition}
\def\corollaryautorefname{Corollary}
\def\questionautorefname{Question}
% rewriting items does not work : ugly hack on content.tex

\newcommand{\intv}[1]{\{1,\dots,#1\}}

\newcommand{\domenum}{\textsc{Dom-Enum}}
\newcommand{\cdomenum}{\textsc{CDom-Enum}}
\newcommand{\tdomenum}{\textsc{TDom-Enum}}
\newcommand{\transenum}{\textsc{Trans-Enum}}
\newcommand{\rbdomset}{\textsc{Red-Blue Dominating Set}}
\newcommand{\grbdomset}{\textsc{Generalized Red-Blue Dominating Set}}

\newcommand{\mcis}{\textsc{Multicolored Independent Set}}

\DeclareMathOperator{\inc}{{\sf inc}}
\DeclareMathOperator{\parent}{{\sf parent}}
\DeclareMathOperator{\children}{{\sf children}}
\DeclareMathOperator{\priv}{{\sf priv}}
\DeclareMathOperator{\Min}{Min}
\DeclareMathOperator{\Max}{Max}

\DeclareMathOperator{\mds}{MDS}
\DeclareMathOperator{\mcds}{MCDS}
\DeclareMathOperator{\mtds}{MTDS}

% Utils packages
\setlength{\marginparwidth}{4cm}
\usepackage[textsize=small, color=black!50, backgroundcolor=white]{todonotes}

\usepackage{tabto} % symbol on margin to help identify changes in addition to color + warning !
\def\marginsymbol{\protect\marginsymbolhelper}
\def\marginsymbolhelper{\tabto*{-1cm}\makebox[0cm]{\scalebox{2}{\texttimes}}\tabto*{\TabPrevPos}}

\newcommand{\todowarn}{\PackageWarning{todonotes}{some todo still there}} % so that we can easily find remaining textcolor
\newcommand{\odtodo}[1]{\todo[backgroundcolor=green!20!white]{#1}}
\newcommand{\gcmgtodo}[1]{\todo[backgroundcolor=orange!20!white]{#1}}
\newcommand{\ectodo}[1]{\todo[backgroundcolor=blue!20!white]{#1}}
\newcommand{\reviewer}[1]{\todo[backgroundcolor=red!20!white]{#1}}

\newcommand{\od}[1]{\textcolor{green!50!black}{\marginsymbol{}#1}\todowarn}
\newcommand{\ec}[1]{\textcolor{blue!70!black}{\marginsymbol{}#1}\todowarn}
\newcommand{\gcmg}[1]{\textcolor{red!70!black}{\marginsymbol{}#1}\todowarn}

% Macros
\def\H{\mathcal{H}}
\def\NN{\mathcal{N}}
\newcommand{\G}{\mathcal{G}}
\def\S{\mathcal{S}}
\def\N{\mathbb{N}}
\def\Z{\mathbb{Z}}
\def\O{\mathcal{O}}

\def\NP{$\mathsf{NP}$}
\def\PNP{$\mathsf{P=NP}$}




\def\PNP{$\mathsf{P=NP}$}
